Fast Adaptive Fourier Integration for Spectral Densities of Gaussian Processes

The specification of a covariance function is of paramount importance when employing Gaussian process models, but the requirement of positive definiteness severely limits those used in practice. Designing flexible stationary covariance functions is, however, straightforward in the spectral domain, where one needs only to supply a positive and symmetric spectral density. In this work, we introduce an adaptive integration framework for efficiently and accurately evaluating covariance functions and their derivatives at irregular locations directly from \textit{any} continuous, integrable spectral density. In order to make this approach computationally tractable, we employ high-order panel quadrature, the nonuniform fast Fourier transform, and a Nyquist-informed panel selection heuristic, and derive novel algebraic truncation error bounds which are used to monitor convergence. As a result, we demonstrate several orders of magnitude speedup compared to naive uniform quadrature approaches, allowing us to evaluate covariance functions from slowly decaying, singular spectral densities at millions of locations to a user-specified tolerance in seconds on a laptop. We then apply our methodology to perform gradient-based maximum likelihood estimation using a previously numerically infeasible long-memory spectral model for wind velocities below the atmospheric boundary layer.

==> figures/lidar_data.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(9070.00,4534.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1682,2380){\makebox(0,0)[r]{\strut{}\tiny -2}}%
      \put(1682,2805){\makebox(0,0)[r]{\strut{}\tiny -1}}%
      \put(1682,3230){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \put(1682,3654){\makebox(0,0)[r]{\strut{}\tiny 1}}%
      \put(1682,4079){\makebox(0,0)[r]{\strut{}\tiny 2}}%
      \put(2842,2160){\makebox(0,0){\strut{}}}%
      \put(3906,2160){\makebox(0,0){\strut{}}}%
      \put(4970,2160){\makebox(0,0){\strut{}}}%
      \put(6034,2160){\makebox(0,0){\strut{}}}%
      \put(7098,2160){\makebox(0,0){\strut{}}}%
      \put(8162,2160){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7175,3906){\makebox(0,0)[r]{\strut{}1.17km}}%
      \csname LTb\endcsname%%
      \put(945,3229){\rotatebox{-270.00}{\makebox(0,0){\strut{}velocity (m/s)}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1682,666){\makebox(0,0)[r]{\strut{}\tiny -3}}%
      \put(1682,878){\makebox(0,0)[r]{\strut{}\tiny -2}}%
      \put(1682,1091){\makebox(0,0)[r]{\strut{}\tiny -1}}%
      \put(1682,1303){\makebox(0,0)[r]{\strut{}\tiny 0}}%
      \put(1682,1516){\makebox(0,0)[r]{\strut{}\tiny 1}}%
      \put(1682,1728){\makebox(0,0)[r]{\strut{}\tiny 2}}%
      \put(1682,1941){\makebox(0,0)[r]{\strut{}\tiny 3}}%
      \put(2842,233){\makebox(0,0){\strut{}\tiny 13.5}}%
      \put(3906,233){\makebox(0,0){\strut{}\tiny 14}}%
      \put(4970,233){\makebox(0,0){\strut{}\tiny 14.5}}%
      \put(6034,233){\makebox(0,0){\strut{}\tiny 15}}%
      \put(7098,233){\makebox(0,0){\strut{}\tiny 15.5}}%
      \put(8162,233){\makebox(0,0){\strut{}\tiny 16}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7175,1980){\makebox(0,0)[r]{\strut{}0.09km}}%
      \csname LTb\endcsname%%
      \put(945,1303){\rotatebox{-270.00}{\makebox(0,0){\strut{}velocity (m/s)}}}%
      \put(4988,-97){\makebox(0,0){\strut{}time (h)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={453.50bp},height={226.70bp}]{./figures/lidar_data}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/lidar_matern_mles.tex <==
 case & $-\ell(\hat{\bth})$ & $\phi$ & $\rho$ & $\nu$ & $p$ & $\tau$ \\ 
 \hline 
Below ABL, $p=0$ & \num{-4.634e+03} & \num{2.828e+01} & \num{1.774e+02} & \num{7.805e-01} & \num{-0.000e+00} & \num{7.589e-08} \\ 
Below ABL        & \num{-4.746e+03} & \num{5.119e+02} & \num{5.308e+02} & \num{8.543e-01} & \num{-6.255e-01} & \num{0.000e+00} \\ 
\hline
Above ABL, $p=0$ & \num{-7.039e+03} & \num{1.523e+02} & \num{3.425e+01} & \num{1.987e+00} & \num{-0.000e+00} & \num{2.687e-01} \\ 
Above ABL        & \num{-7.040e+03} & \num{1.651e+01} & \num{9.947e+01} & \num{8.800e-01} & \num{-8.926e-01} & \num{2.684e-01} 


==> figures/singular_matern_compare.tex <==
&\multicolumn{4}{c|}{double precision} & \multicolumn{4}{c|}{extended precision} & \multicolumn{4}{c|}{our method} \\ 
\hline 
& time (s) & $|K(1/2)|$ & $|K(1)|$ & $\lambda_{\text{min}}(\bm{\Sigma}) $ & time (s) & $|K(1/2)|$ & $|K(1)|$ & $\lambda_{\text{min}}(\bm{\Sigma}) $ & time (s) & $|K(1/2)|$ & $|K(1)|$ & $\lambda_{\text{min}}(\bm{\Sigma}) $ \\ 
$\rho=2$ & \num{4.726e-04} & \num{1.948e-01} & \num{1.017e-01} & \num{-1.208e-08} & \num{1.825e+01} & \num{1.948e-01} & \num{1.017e-01} & \num{3.230e-11} & \num{9.260e-01} & \num{1.948e-01} & \num{1.017e-01} & \num{2.931e-11}  \\ 
$\rho=4$ & \num{4.350e-04} & \num{1.017e-01} & \num{5.922e-02} & \num{-1.556e-02} & \num{1.860e+01} & \num{1.017e-01} & \num{6.148e-02} & \num{7.312e-10} & \num{9.825e-01} & \num{1.017e-01} & \num{6.145e-02} & \num{7.305e-10}  \\ 
$\rho=6$ & \num{5.078e-04} & \num{7.546e-02} & \num{2.373e+03} & \num{-1.980e+04} & \num{1.885e+01} & \num{7.547e-02} & \num{2.180e+01} & \num{-2.497e+02} & \num{9.128e-01} & \num{7.547e-02} & \num{4.613e-02} & \num{4.533e-09}  \\ 
$\rho=8$ & \num{5.707e-04} & \num{5.866e-02} & \num{1.507e+09} & \num{-6.930e+09} & \num{1.904e+01} & \num{6.148e-02} & \num{1.006e+07} & \num{-1.018e+08} & \num{1.118e+00} & \num{6.145e-02} & \num{3.768e-02} & \num{1.654e-08}  \\ 
$\rho=10$ & \num{6.412e-04} & \num{1.350e+00} & \num{6.758e+14} & \num{-2.516e+15} & \num{1.923e+01} & \num{8.240e-02} & \num{4.165e+12} & \num{-3.438e+13} & \num{9.042e-01} & \num{5.246e-02} & \num{3.222e-02} & \num{4.513e-08}  \\ 


==> src/singular.tex <==

Before applying our numerical approach to compute MLEs from data, we establish
a theoretical result regarding the general class of spectral densities with
origin singularities of the form $|\omg|^{-\alpha} S(\omg)$, where $S$ is a
bounded, integrable spectral density. Despite the popularity of special cases of
these long-memory models in time series applications \citep{brockwell1991time},
to our knowledge they are rarely used in continuous-time settings. 
%This is no
%doubt due in part to the numerical challenges addressed in the previous section,
%and we provide the following theorems to underscore the useful properties of
%this model class, which can now be efficiently numerically evaluated using our
%method. All proofs for the theorems in this section can be found in the online
%supplement.
%
%While there remain a great number of non-singular spectral densities whose
%Fourier transforms cannot be computed in closed form, we demonstrate in this
%section that singularities provide a valuable degree of freedom when writing
%parametric families of covariance functions. 
%
%First, we show that the exponent $\alpha$ of an integrable singularity is
%``microergodic" in some fixed-domain asymptotic settings. Formally, for a
%parametric family of Gaussian measures $\set{P_{\bth}}_{\bth \in \bm{\Theta}}$,
%a quantity $h(\bth)$ is microergodic if $h(\bth) \neq h(\bth')$ implies
%$P_{\bth} \perp P_{\bth'}$ in the sense that there exists an event $A$ such that
%$P_{\bth}(A) = 0$ and $P_{\bth'}(A) > 0$.  Practically, the significance of this
%concept is that microergodic quantities can be estimated consistently from just
%one sample path of a Gaussian process \citep{stein1999interpolation}. 
%The microergodicity of $\alpha$ may be a somewhat surprising conclusion, as in
%most fixed-domain asymptotic settings in dimension $d < 4$, covariance model
%parameters are not typically consistently estimable individually
%\citep{stein1999interpolation,zhang2004inconsistent}. As the following theorem
%demonstrates, however, for singular spectral densities one can construct
%quadratic forms which have finite expectation for a given $\alpha$ and infinite
%expectation for any $\alpha' > \alpha$, effectively distinguishing the two
%measures. 
%The implication of this theorem --- that $\alpha$ can be estimated well from
%data --- is validated by the application shown in the following section. 
%
%\begin{theorem} \label{thm:microergodic}
%Let $S_{\bth} \in L^1(\R)$ be a bounded, symmetric, positive spectral density
%for all $\bth \in \bm{\Theta}$, and take $\alpha \in [0,1)$. Let $P_{\alpha,
%\bth}$ be the measure corresponding to the spectral density $|\omega|^{-\alpha}
%S_{\bth}(\omega)$. Then the parameter $\alpha$ is microergodic in the family of
%models $\set{P_{\alpha, \bth} \sv (\alpha, \bth) \in [0,1) \times \bm{\Theta}}$
%for processes defined on a finite interval $T$.
%\end{theorem}
%
An interesting property of singular spectral densities is that they can be
used to build covariance functions that decay exceptionally slowly.  
% So-called ``long-memory" processes in time series use, for example,
% singularities with $0 \leq \alpha < \frac{1}{2}$ \citep{brockwell1991time}. 
In the following theorem we provide tail decay rates for all integrable
singularities $\omega^{-\alpha}$, and show that one can obtain covariance
functions of arbitrarily slow power law asymptotic decay.

\begin{theorem} \label{thm:decay} Let $S \in C^2(\R) \cap L^1(\R)$ be a bounded,
  symmetric, positive spectral density with $S', S'' \in L^1(\R)$. Then for all
  $\alpha \in [0,1)$
  \begin{equation*} %\label{eq:}
    K_\alpha(r) 
    := 2\int_0^\infty |\omega|^{-\alpha} S(\omega) \cos(2 \pi \omega r) \dif \omega 
    \sim r^{-1+\alpha} \quad \text{as} \ r \to \infty.
  \end{equation*}
\end{theorem}

The requirement $S \in C^2(\R)$ is far from a necessary condition, and this
asymptotic behavior is a very general phenomenon. For example $S(\omega) =
\expp{-\abs{\omega}}$ yields the covariance function 
\begin{align}
  K_\alpha(r)
  % &:= \Fr^{-1}\left\{\abs{\omega}^{-\alpha} \expp{-\abs{\omega}}\right\} \\
  & = \frac{2}{\Gamma(1-\alpha)} \Big( 1 + (2\pi r)^2 \Big)^{-\frac{1}{2}(1-\alpha)} \cos\Big((1-\alpha) \tan^{-1}(2\pi\abs{r})\Big)
  \sim r^{-1+a}
\end{align}
as $r \to \infty$ despite the fact that $S$ is not even $C^1(\R)$. In such cases
one can apply more general Tauberian results from the theory of slowly varying
functions to obtain the same asymptotic decay \cite[Theorem
4.10.3]{bingham1989regular}. We note, however, that this result trades
smoothness for monotonicity requirements in $S$. \blue{Our result, which is
proved using elementary properties of convolutions, is applicable to a
comparatively large class of models.}
%Therefore, we find that our above elementary proof demonstrates a useful
%connection to convolutions, and is applicable to a large class of spectral
%densities relevant to the current work.



==> src/twodim.tex <==

\red{This is just a placeholder so I don't mess up the git history of any of the
files we have agreed on or you have any stashed work on.}

\bigskip

By the standard change-of-variables of $\bx = (\rho \cos \psi, \rho \sin \psi)$
and $\bm{\omg} = (r \cos \theta, r \sin \theta)$, the two-dimensional Fourier
transform of a spectral density $S(\bm{\omg})$ can be written as
\begin{equation*} %\label{eq:}
  \int_{\R^2} e^{2 \pi i \bm{\omg}^T \bx} S(\bm{\omg}) \dif \bm{\omg}
  =
  \int_{0}^{\infty} \int_{-\pi}^{\pi} S(r, \theta) e^{2 \pi i \rho r \cos(\theta
  - \psi)} \dif \theta \dif r.
\end{equation*}
Or maybe there is a $2 \pi$ that I missed somewhere, but whatever. The idea is
very simple: if the SDF in polar coordinates $S(r, \theta)$ is very smooth in
$\theta$ marginally for each $r$, then one can very accurately discretize the
inner integral and obtain (after applying Fubini-Tonelli) that
\begin{equation} \label{eq:appx_2dft}
  \int_{0}^{\infty} \int_{-\pi}^{\pi} S(r, \theta) e^{2 \pi i \rho r \cos(\theta
  - \psi)} \dif \theta \dif r 
  \approx
  \sum_{l=1}^{L} w_l 
  \int_{0}^{\infty} S(r, \theta_l) e^{2 \pi i \rho r
  \cos(\theta_l - \psi)} \dif r.
\end{equation}
But that RHS equation is nice because $\theta_l$ is fixed! If the locations you
need the kernel at are $\set{\bx_j}_{j=1}^n$, which in polar coordinates
corresponds to $\set{(\rho_j, \psi_j)}_{j=1}^n$, you just need (for each $l$!)
to use our \texttt{kernel\_values} code with integrand $r \mapsto S(r,
\theta_l)$ at frequencies $\set{\rho_j \cos(\theta_l - \psi_j)}_{j=1}^n$. And
then you simply sum the values across the $l$ index and obtain the finalized
Fourier transform. But if $S(r, \theta)$ is smooth in $\theta$ for each $r$,
then maybe $L=32$ or something would be good enough. 

\bigskip

There is only one item that would need to change about \texttt{kernel\_values},
which is that we would want it to be able to take negative $x$ values or handle
the symmetry correctly. But it seems unthinkable that that would be a real
issue.

\bigskip
\bigskip

I like this idea because to some degree it is dumb and obviously improvable, so
it doesn't really rule out the next paper. But if we could even just generate
some plots of the implied kernels that we can dream up with these spectral
domain deformations, I think a few mind blowing plots and then saying ``but this
clearly requires more R\&D" could help sell this project.



